New Approaches for Quantum Copy-Protection

Quantum copy protection uses the unclonability of quantum states to construct quantum software that provably cannot be pirated. Copy protection would be immensely useful, but unfortunately little is known about how to achieve it in general. In this work, we make progress on this goal, by giving the following results: - We show how to copy protect any program that cannot be learned from its input/output behavior, relative to a classical oracle. This improves on Aaronson [CCC'09], which achieves the same relative to a quantum oracle. By instantiating the oracle with post-quantum candidate obfuscation schemes, we obtain a heuristic construction of copy protection. -We show, roughly, that any program which can be watermarked can be copy detected, a weaker version of copy protection that does not prevent copying, but guarantees that any copying can be detected. Our scheme relies on the security of the assumed watermarking, plus the assumed existence of public key quantum money. Our construction is general, applicable to many recent watermarking schemes.

==> acknowledge.tex <==

\section*{Acknowledgements}

We thank Paul Christiano for suggesting the idea of quantum copy-protection based on \cite{aaronson2012quantum} hidden subspace oracles.

%Scott Aaronson for the inspiring discussion, his guidance on this project and great comments on this paper

==> moneyfromcopy.tex <==
\section{Public Key Quantum Money from Copy Protection}
%\Jiahui{change the use of testing distribution to joint distribution}


Quantum copy-protection and quantum money are closely related. In this section, we give two constructions from general quantum copy-protection scheme
to build public-key quantum money: one using a CCA2-secure public-key encryption scheme (\cref{thm:money_from_pke,thm:money_from_pke_2}); one using a trapdoor function (\cref{thm:money_from_trapdoor}). The construction based on CCA2-secure PKE has a reliable post-quantum PKE primitive based on LWE problem; on the other hand, the construction from trapdoor functions may be more lightweight due to simpler underlying primitives.

We also point out that the notion of public-key unclonable decryption keys in \cite{georgiou-zhandry20} (who came out a little later than the first verision of this paper) can be seen as a copy-protection of decryption functions.
 
%Without specification, the quantum copy-protection scheme used refers to a general quantum copy protection for all quantumly unlearnable functions.   

%we need currently have no provably secure constructions from standard post-quantum assumptions

\iffalse
An inverse of a trapdoor \cref{def:trapdoor} is hard to compute without the trapdoor. Therefore, a quantum-secure trapdoor function's inverse cannot be computed efficiently for any %QPT adversary. 
If there exists any QPT adversary which can learn the inverse of a trapdoor function with only oracle access, then it can be used to compute the function efficiently without a trapdoor, contradicting the property of trapdoor functions. \Jiahui{Not necessarily? }
Therefore, any family of quantum-secure trapdoor functions (inverses) are quantumly unlearnable and can be copy-protected. 
\fi


\subsection{Public-Key Quantum Money from CCA-secure Public-Key Encryption}

We give the definition of a public-key encryption scheme and CCA2 security (often simply referred to as CCA security) in \cref{def:pke}. Quantum CCA-security was studied in \cite{bonehzhanz2013quantumMAC} where the adversary can make quantum superposition queries to the encryption and decryption oracles.
%By our definition of quantum copy protection security and quantum unlearnability, the oracle queries are classical and the programs can also only output classical computation results; therefore, we can consider a notion of ``weak quantum CCA security" where the QPT adversary has quantum resources but only queries the encryption and decryption oracles classically. The weak quantum CCA-security definition will be the same as given in \cref{def:pke} except that the adversary is QPT.


\paragraph{CCA-secure PKE Schemes} \cite{bonehzhanz2013quantumMAC} presents a proof that public-key quantum CCA security can be obtained from any identity-based encryption scheme that is selectively secure under a quantum chosen identity attack and
such an identity-based encryption scheme can be built from lattice assumptions, specifically the Learning With Errors (LWE) assumption (\cref{def:lwe}). 
Another candidate scheme is a CCA-secure McEliece
based public-key cryptosystem  in the standard model from \cite{dottling2012cca2-mceliece}, since McEliece public-key cryptography is yet known to be broken by quantum adversaries either.

The goal of this section is to prove the following theorems. By assuming post-quantum CCA-secure public-key encryption scheme, we have \cref{thm:money_from_pke}. And by assuming the quantum resistance of LWE, we have \cref{thm:money_from_pke_2}.
\begin{theorem}
\label{thm:money_from_pke}
Assume that there exists a post-quantum CCA-secure public-key encryption scheme and there exists a secure quantum copy-protection scheme for decryption functions of such CCA-secure public-key encryption scheme, then there exists a secure public-key quantum money scheme.
\end{theorem}


\begin{theorem}
\label{thm:money_from_pke_2}
Assume that the Learning With Errors problem with certain parameters is hard for $QPT$ adversaries and there exists a secure quantum copy-protection scheme for decryption functions of LWE-based CCA-secure public-key encryption schemes, then there exists a secure public-key quantum money scheme.
\end{theorem}



\subsubsection{Public-key Quantum Money Scheme}
We first state the construction of the public-key quantum money.
Assume that we have an underlying public key encryption scheme called $\pke = (\pke.\keygen, \pke.\enc, \pke.\enc)$, whose description and the message space $\cM$ are public. 
%The public-key quantum money scheme I is as follows:

\begin{figure}[H]
    \centering
    \begin{gamespec}
    \begin{description}
    \item $\keygen(1^\lambda) \to (\pk,\sk):$ takes in security parameter $n$; run $\pke.\keygen(1^\lambda) \to (\pke.\pk, \pke.\sk)$. 
    It also generates a testing parameter $k = \poly(\lambda)$. 
    
    Outputs $\pk = (\pke.\pk, k)$ and $\sk = \pke.\sk$.
    
    \item $\gennote(\sk) \to \ket{\$}:$ takes in the secret key; and runs $\textsf{Generation}$ algorithm of $\cp$ for the decryption function $\pke.\dec(\pke.\sk, \cdot)$ to generate $\cp(\pke.\dec(\pke.\sk, \cdot))$.
    
    Outputs $\ket{\$} = \cp(\pke.\dec(\pke.\sk, \cdot))$.
    
    \item $\ver(\pk, \ket{\$}) \to 0/1:$  takes in the public key $\pk = (\pke.\pk, k)$ and a claimed banknote state $\ket{\$} = \P$, i.e. a claimed copy-protection program for $\pke.\dec(\pke.\sk, \cdot)$. First, it samples $k$ number of uniformly random $m_i \gets \cM$, compute $c_i = \pke.\enc(\pke.\pk, m_i)$, for each $i \in [k]$. Next, runs $\P$ on $c_i$ and checks if $\P(c_i) = m_i$, for each $i \in [k]$; if all of the evaluations are equal, output 1 for accept, otherwise 0 for reject. 
    \Jiahui{verify by Check and ATI}
    \end{description}
    \end{gamespec}
    \caption{Public-key Quantum Money Scheme I.}
    \label{fig:pk_money_I}
\end{figure}
\subsubsection{Security Analysis}
We now show that the construction is secure based on the assumptions of \cref{thm:money_from_pke} and \cref{thm:money_from_pke_2}.
\begin{proof}[Proof of \cref{thm:money_from_pke}]
The construction of the public-key quantum money is stated in \cref{fig:pk_money_I}. The security of the scheme follows from   \cref{lem:money_pke_secure}. \qed
\end{proof}

\cref{thm:money_from_pke_2} has the same construction of quantum money scheme. The security follows from the same proof of \cref{thm:money_from_pke}, and we omit it here.  
\paragraph{Verification Correctness}
\begin{lemma}
The public-key quantum money construction in \cref{fig:pk_money_I}
satisfies verification correctness. \end{lemma}
\begin{proof}
By the computation correctness of the underlying copy-protection $\cp$ and decryption correctness of the underlying $\pke$, a valid banknote $\ket{\$} = \cp(\pke.\dec(\pke.\sk, \cdot))$ is supposed to compute $\pke.\dec(\sk, c)$ on a ciphertext $c = \pke.\enc(\pke.\pk, m)$ for any $m \in \cM$ correctly, with all but negligible probability over the generation of keys $(\pke.\pk, \pke.\sk)$. Therefore, verification correctness holds. \qed
\end{proof}

\paragraph{Unclonable Security} We  give a brief proof for the unclonable security of the quantum money scheme, whose security definition is given in \cref{def:money}. Our goal is to copy-protect the decryption function hard-coded with a secret key $\pke.\dec(\pke.\sk, \cdot)$, where $\pke.\sk \gets \pke.\keygen(1^\lambda)$.

\begin{claim}
\label{claim:cca_unlearnable}
Assuming that $\pke$ is quantum CCA-secure, the family of decryption functions $\pke.\dec \\ (\pke.\sk, \cdot)$, where $(\pke.\sk,\pke.\pk) \gets \pke.\keygen(1^\lambda)$ is quantumly unlearnable, and the challenger tests on inputs that are encryptions of uniform random messages from message space using the corresponding public key $\pk$.
\end{claim}

\begin{proof}
Suppose there exists some QPT adversary $\cA$ for which the decryption function family is quantumly learnable, then we can construct a QPT adversary $B$ who can break weak quantum CCA security. 

After the setup phase, $B$ passes public information it receives from the challenger to $\cA$.  During the query phase of CCA security game, $B$ simply passes $\cA$'s computation queries on $c$ to the decryption oracle; the oracle will return $m$ or $\bot$ and $B$ sends the reply to $\cA$. During challenge phase, $B$ chooses uniform random messages $m_0, m_1 \gets \cM$ and queries the encryption oracle to get a challenge ciphertext $\ct = \enc(\pk, m_b)$. $B$ does the same thing during the query phase after challenge as the query phase before.  After $\cA$ goes into its challenge phase, it will provide a quantum circuit $C$ that supposedly computes $\dec(\sk, \cdot)$. $B$ applies $C$ on $\ct$ and gets $m_b'$. If $\cA$ has non-negligible advantage $\epsilon$ in successfully learning $\pke.\dec(\sk, \cdot)$, then we have $m_b' = m_b$ with probability $\epsilon$. Therefore, $B$ breaks weak quantum CCA security with advantage $\epsilon$. \qed
\end{proof}
 
%We conjecture that there exists copy protection scheme for decryption function with respect to this testing distribution $\cD_u$, the same distribution used in $\ver$ of the quantum money scheme.
%\Ruizhe{Can we remove this conjecture? Or we should state it in the following lemma and the \cref{thm:money_from_pke} as an additional assumption.}

\begin{lemma}
\label{lem:money_pke_secure}
Assuming that $\pke$ is quantum CCA-secure and there exists a secure quantum copy-protection scheme $\cp$ for $\{\pke.\dec(\sk, \cdot): (\pke.\sk,\pke.\pk) \gets \pke.\keygen(1^\lambda) \}$, then public-key quantum money scheme I has unclonable security.
\end{lemma}

\begin{proof}
%By \cref{claim:cca_unlearnable}, if $\pke$ is quantum CCA-secure,  we assume the existence of a general copy-protection scheme for quantumly unlearnable functions.
Suppose there is a QPT adversary $\cA$ that breaks unclonable security, then we can construct a QPT adversary $B$ that breaks anti-piracy security for $\cp$. 


The quantum copy protection challenger will copy-protect a decryption function of $\pke$: it first runs the  setup $\pke.\keygen$ and publishes the public key $\pk$; then generates $k$ copies of copy protection program $\{\cp_i(\dec(\sk, \cdot))\}_{i \in [k]}$ and gives them to $B$. Then $B$ sends $\pk$ to $\cA$ as the public key for quantum money and $\{\cp_i(\dec(\sk, \cdot))\}_{i \in [k]}$ as $k$ money states $\{\ket{\$}\}_{i \in [k]}$. Finally, $\cA$ output $k+1$ number of claimed money states $\{\rho_i\}_{i \in [k+1]}$ and sends to $B$. $B$ uses them as its pirate programs and passes to copy-protection challenger. Since the testing distributions for the money states and copy protection of $\pke.\dec$ are the same, if $\cA$ has non-negligible advantage $\epsilon$, then $B$ has non-negligible advantage $\epsilon$.
\end{proof}

\paragraph{Unclonable Decryption Keys and Copy-Protection for Decryption}

Unclonable decryption keys, or single-decryptor encryption scheme is a new notion from \cite{georgiou-zhandry20}.
The high level idea is that the encryption scheme allows an authorized user to decrypt messages by issuing him a quantum state as his decryption key; the user can then decrypt ciphertexts encrypted with the corresponding encryption key; however,the user cannot share this secret key with someone else so that both of them can decrypt ciphertexts at the same time.

Here we briefly discuss the relationship of this notion with copy-protection of decryption functions. 
%we first present the definition for single-decryptor encryption below.






\subsection{Public-key Quantum Money from Trapdoor Functions}
 
 We first present the definition of
 trapdoor functions.
 \begin{definition}[Injective Trapdoor Functions]
\label{def:trapdoor}
An injective trapdoor function funmily $\tdf$ with input space $\{0,1\}^n$ and output $\{0,1\}^m$, where $m,n = \poly(\lambda)$ consists of the following algorithms:
\begin{itemize}
    \item $\tdf.\setup(1^\lambda) \to (\tdf.\pk, \tdf.\sk$): The setup algorithm takes as input security
parameter $\lambda$ and outputs a public key $\tdf.\pk$ and secret key $\tdf.\sk$.

    \item $\tdf.\eval(\tdf.\pk, x \in \{0,1\}^n) \to y$: The evaluation algorithm takes as input
an input $x \in \{0,1\}^n$ and public key $\tdf.\pk$, and outputs $y \in \{0, 1\}^m$.


\item $\tdf.\invert(\tdf.\sk, y \in \{0,1\}^m) \to x/ \bot$: The inversion algorithm takes as input $y \in \{0, 1\}^m$ and secret key $\tdf.\sk$, and outputs $x$, which is
either $\bot$ or a $n$-bit string. 

    

\end{itemize}

An injective trapdoor function family should satisfy the following properties:

\textbf{Almost-All-Keys Injectivity}.  We require that for nearly all public/secret keys,
inversion works for all inputs. More formally, there exists a negligible function $\negl(\cdot)$ such that for all $\lambda \in \N$:
\begin{gather*}
    \Pr\left[\exists x \text{ s.t. } \tdf.\invert(\tdf.\eval(\tdf.\pk, x),\tdf.\sk) \neq x \right] \leq \negl(\lambda) 
\end{gather*}




\textbf{Hard-to-Invert}. A trapdoor family is hard-to-invert if for any PPT
adversary $\cA$, there exists a negligible function $\negl(\cdot)$ such that for all $\lambda \in \N$:
\begin{gather*}
  \Pr\left[ x \gets \cA(\tdf.\pk, y): 
    \begin{array}{cl}
      (\tdf.\pk,\tdf.\sk) \gets \tdf.\setup(1^\lambda)\\
      x \gets \{0, 1\}^n , y = \tdf.\eval(\tdf.\pk, x)
    \end{array}
  \right] \leq \negl(\lambda).
\end{gather*}


%a one-way function family and we can sample $f \gets \cF$ together with a trapdoor $t$, so that for any PPT algorithm $A$:$$\Pr[A(t, f(x)) \in f^{-1}(f(x))] = 1$$

\end{definition}



 The family of trapdoor functions we need for our construction requires one more property, in addition to  \cref{def:trapdoor}: 
\begin{itemize}
    %\item \textbf{Injective:} we need these trapdoor functions to be injective so that their inverses can be computed correctly and anyone can verify them with only negligible error.
    
%    \item \textbf{Uniform testing distribution:} for an injective trapdoor function $f \in \cF: \cal X \to \cal Y$, we can verify, using a testing distribution $\cD_u$, if a program $\P$ is a copy-protection program for inversion function with hard-coded trapdoor $\tdf.\invert(\tdf.\sk, \cdot)$, where $\tdf.\sk$. The testing inputs in $\cD_u$ is obtained by sampling uniformly random $x \gets \cal X$ and computing $y = f(x)$. Then the verification is to check if $\P(y) = x$. 
    
    \item \textbf{Quantum unlearnability of inversion:} for a family of injective trapdoor functions $\tdf$ with input space $\{0,1\}^n$ and output space $\{0,1\}^m$,  its inversion functions hard-coded with a secret key:
    $$
    \left\{\tdf.\invert(\tdf.\sk, \cdot): \begin{array}{cl}(\tdf.\pk,\tdf.\sk) \gets  \tdf.\setup(1^\lambda) \\
    \forall x \in \{0,1\}^n, \tdf.\invert(\tdf.\sk, \tdf.\eval(\tdf.\pk, x)) = x
    \end{array}\right\}
    $$
    is quantumly unlearnable, the adversary's winning probability taken over the choice of $(\tdf.\pk,\\ \tdf.\sk)$ and uniformly random $x \in \{0,1\}^n$.
    
\end{itemize}

For rest of this section, we will refer to these inversion functions $\{\tdf.\invert(\tdf.\sk, \cdot)\}$ where the corresponding trapdoor function $\cF$ satisfies the above properties, as inverse trapdoor functions for short. 

Post-quantum injective trapdoor functions can also be instantiated with LWE. However, this additional property is not trivial to achieve: inversion of trapdoor functions cannot be computed efficiently by their one-wayness, but giving the adversary an inversion oracle is more power; we will give some discussions on candidate trapdoor functions.
%Many existing trapdoor function constructions satisfy the injective property and uniform testing distribution property. 

%In \cref{sec:lwe_trapdoor} we will show that a candidate a trapdoor function built from lattice-based assumptions that may satisfy these requirements.
The goal of this section is to prove \cref{thm:money_from_trapdoor}.
\begin{theorem}
\label{thm:money_from_trapdoor}
If there exists quantum-secure injective trapdoor functions that satisfy unlearnability of its inversion functions, and there exists a secure quantum copy-protection scheme for its inversion functions, then there exists a secure public-key quantum money scheme.
\end{theorem}

\subsubsection{Public Key Quantum Money Scheme II} 
Our construction of public key quantum money scheme II is as follows. We assume that we already have an underlying quantum copy-protection scheme $\cp$ and we have a trapdoor function family $\tdf$.

%The $\keygen$ algorithm is slightly different from \cref{def:money} in that it takes in a description of a trapdoor function family $\cF$. .
\begin{figure}[H]
    \centering
    \begin{gamespec}
    \begin{description}
    \item $\keygen(1^\lambda) \to (\pk, \sk):$ takes in security parameter $\lambda$; run $\tdf.\setup(1^lambda) \to (\tdf.\sk, \tdf.\pk)$; generate a testing parameter $k = \poly(n)$. 
    %a description of a trapdoor function family $\cF: \{0.1\}^m \to \{0,1\}^l, m,l = \poly(n)$
    
    
    Outputs $\pk = (k, \tdf.\pk)$ and $\sk = \tdf.\sk$. %where $f(\cdot)$ and $g(t, \cdot)$ are presented in descriptions.
    
    \item $\gennote(\sk) \to \ket{\$}:$ takes in the secret key $\sk = \tdf.\sk$ and runs $\textsf{Generation}$ algorithm of $\cp$ to generate $\cp(\tdf.\invert(\tdf.\sk, \cdot))$, a copy-protection program for $\tdf.\invert(\tdf.\sk, \cdot)$. 
    
    Outputs $\ket{\$} = \cp(\tdf.\invert(\tdf.\sk, \cdot))$.
    
    \item $\ver(\pk, \ket{\$}) \to 0/1:$  takes in the public key $\tdf.\pk$, testing parameter $k$ and a claimed banknote state $\ket{\$} = \P$, i.e. a claimed copy-protection program for $\cp(\tdf.\invert(\tdf.\sk, \cdot))$. It samples $k$ number of uniformly random $x_i \gets \{0,1\}^n$, compute $y_i = \tdf.\eval(\tdf.\pk, x_i)$, for each $i \in [k]$. Next, runs $\P$ on $y_i$ and checks if $\P(y_i) = x_i$ for each $i \in [k]$; if all of the evaluations are equal, output 1 for accept, otherwise 0 for reject.
    \end{description}
    \end{gamespec}
    \caption{Public Key Quantum Money Scheme II.}
    \label{fig:pk_money_II}
\end{figure}
\subsubsection{Security Analysis}
\paragraph{Verification Correctness:} 
By the computation correctness of the underlying copy-protection $\cp$, a valid banknote $\ket{\$} = \cp(\tdf.\invert(\tdf.\sk, \cdot))$ is supposed to compute $\tdf.\invert(\tdf.\sk, \cdot))$ on any valid $y = \tdf.\eval(\tdf.\sk, x)$ correctly, with all but negligible probability. Therefore, verification correctness holds.


\paragraph{Unclonable Security}
\begin{claim}
\label{claim:money_trapdoor_secure}
Assume that there exists a secure quantum copy-protection scheme $\cp$ for the injective trapdoor funciton family $\tdf$ with quantum unlearnable inversion function,  then public key quantum money scheme II has unclonable security.
\end{claim}

Since the inversion functions have quantum unlearnability, the proof idea is the same as \cref{lem:money_pke_secure} except by replacing the copy-protected function with $\tdf.\invert(\tdf.\sk, \cdot)$ and the public key with $\tdf.\pk$. We omit the proof here. 






\paragraph{Discussions on Candidate Trapdoor Functions:}
\label{sec:lwe_trapdoor}
A candidate trapdoor function built from the Learning With Errors (LWE) assumption is the injective trapdoor function in \cite{GPV08} using a Type-I or a \cite{micciancio2012trapdoors} lattice trapdoor . It satisfies the first two properties we need.


One question remains whether its inverse function has the property of being quantumly unlearnable.  \cite{regev2010learning} shows that if the oracle to compute the inverse of this LWE trapdoor function can answer superposition queries and give superpostion outputs, then an efficient quantum attack to find out the trapdoor exists. However, the oracle in the quantum learnability challenge can be only interacted with classically; the copy protection program is also defined to have no superposition output for the underlying function copy-protected. \cite{regev2010learning} also mentioned the difficulty of finding a trapdoor when no superposition queries can be made and if the inputs for the inverse function are required to be valid outputs of the trapdoor function; but no provable hardness is known.

Another option is to investigate trapdoor functions built from other post-quantum primitives such as code-based cryptography.





%In our oracle-setting quantum copy protection construction, we use the same subspace membership oracles as in \cite{aaronson2012quantum}. 

\begin{remark}[Trivial Private Quantum Money Implication]
It is easy to see that quantum copy-protection for any unlearnable functions will imply private-key quantum  money: just let the money issuing authority verify a money state like verifying a pirate program. The testing distribution for many families of functions must be private(e.g. point functions or evasive functions) and otherwise important information about the functions protected would leak. But even for balanced functions with uniform testing distributions that can be public, such as PRF, the verifier still needs to have the same copy-protection program by itself in order to verify a computation, which makes much less sense.
Therefore, this implication from copy-protection to public-verifiable quantum money is not easily realizable without the idea of using a trapdoor or a public key/private key pair.
\end{remark}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
We consider two basic properties of quantum money:
\begin{itemize}
    \item Public verifiable
    \item Non-clonable
\end{itemize}

Then, let $f$ be a quantum-secure trap-door function and suppose it can be quantum copy-protected. Let $(\cp(f),\ket{A})$ be the protected program. Since it is a trap-door function, everyone can verify the correctness of $\cp(f)^\cO(x)$ for any input $x$. Also, by the security of quantum copy-protection scheme, no one can copy $(\cp(f),\ket{A})$ in quantum polynomial-time. Further, since $f$ is a trap-door function, it is certainly non-learnable even for quantum polynomial-time adversaries. Therefore, this scheme satisfies the two properties of quantum money and can be used as a public-key quantum money scheme. 

%\iffalse
\Ruizhe{TODO: Give an explicit algorithm for verification. I guess we can let the verifier randomly pick an input $x$ and compute $\cp(f)(x)$. Then, the verifier can use the trap-door to verify whether the value is correct. We need to show that, for any attack, either on copy-protection scheme or on trap-door function, can only correctly compute a negligible fraction of inputs.}
\fi

==> new_copy_protect_def.tex <==
\subsection{Quantum Copy Protection}

\begin{definition}[Quantum Copy Protection]
\label{def:qcp}

Consider a family of functions $\cF = \{\cF_\lambda: [N_\lambda] \to [M_\lambda]\}$, a quantum copy-protection scheme for
$f \gets \cF_\lambda$ consists of the following procedures:

%\mathcal{X} \rightarrow \mathcal{Y}

%\{0, 1\}^n \rightarrow \{0, 1\}^m

\begin{description}
    \item[]\setup$(1^\lambda) \to (\sk)$: the setup algorithm takes in a security parameter $\lambda$ in unary and generates a secret key $\sk$. 
    
    \item[] \generate$(\sk, f) \rightarrow (\rho_f, \{U_{f, x}\}_{x \in [N]})$:
    on input $f \in \cF_\lambda$ and secret key $\sk$, the vendor generates a quantum program (with classical inputs) $(\rho_f, \{U_{f, x}\}_{x \in [N]})$. %where $U_{f, x}$ is efficiently computable given $x$.  

 \item[]\compute$ (\rho_f, \{U_{f, x}\}_{x \in [N]}) \rightarrow y $:
     given the quantum program, a user can compute the function $f(x)$ for input $x$ by applying $U_{f, x}$ on $\rho$ and measuring the first register of the state. 
\end{description}
\end{definition}

\begin{description}
 \item[] \textbf{Efficiency:}  \textsf{Setup}, $\compute$ and \textsf{Generate}  should run in  $\poly(\lambda)$ time. 
 
    \item[] \textbf{Correctness:}  
   % \begin{itemize}
     %   \item         
     For all $\lambda \in \N$, any $f \in \cF_\lambda$, there exists a negligible function $\neglfunc(\lambda)$ such that for all $x \in [N]$: 
     %the customer can compute the function $f$ correctly %for any QPT customer
     %there exists an QPT algorithm \textsf{Compute} such that
    \begin{align*}
    \Pr\left[\textsf{Compute}(\rho_f, \{U_{f, x}\}_{x \in [N]}, x)=f(x) \,:\, \substack{ \sk \gets \setup(1^\lambda) \\ (\rho_f, \{U_{f, x}\}_{x \in [N]}) \gets \generate(\sk, f)}  \right] \geq 1-\neglfunc(\lambda)
    \end{align*}    
    
    Note that from the Gentle Measurement Lemma (\cref{lem:gentle_measure}), the program can be evaluated polynomially many times on any inputs. 
    
    \item[] \textbf{Security}: It has $\gamma$-anti-piracy security defined below. 
\end{description}



\begin{definition}[$\gamma$-Anti-Piracy Security Game]
An anti-piracy security game for function family $\cF = \{\cF_\lambda: [N] \to [M]\}$, distribution $\cD$ and adversary $\cA$ is denoted as $\AG_{\cF, \cD, \gamma}^\cA(1^\lambda)$, which consists of the following steps:

\begin{enumerate}
    \item \textbf{Setup Phase}: At the beginning of the game, the challenger takes a security parameter $\lambda$ and obtains secret key $\sk \gets \setup(1^\lambda)$.
    
    \item \textbf{Sampling Phase}: The challenger  samples a function $f \gets \cF_\lambda$. 
    
    
    \item \textbf{Query Phase}:
    $\As$ makes a single query to the challenger and obtains a copy-protected program for $f$: $(\rho_f, \{U_{f, x}\}_{x \in [N]}) \gets \generate(\sk, f)$.
    \Qipeng{I made this change because it can be easily extended to $q$-collusion resistant. Just allow $q$ queries in this phase. }
    
    %$\As$ then gets oracle access to $f$;
    \item \textbf{Output Phase}: Finally, $\As$ outputs a (possibly mixed and entangled) state $\sigma$ over two registers $R_1, R_2$ and two sets of unitaries $(\{U_{R_1, x}\}_{x \in [N]}, \{U_{R_2, x}\}_{x \in [N]})$. This can be viewed as two quantum programs $\P_1 = (\sigma[R_1], \{U_{R_1, x}\}_{x \in [N]})$ and $\P_2 = (\sigma[R_2], \{U_{R_2, x}\}_{x \in [N]})$.
    %(i.e. Hilbert spaces $\cH_{R_1},\cH_{R_2}$)
\end{enumerate}
The game outputs $0$ if and only if \emph{both} programs $\P_1, \P_2$ are tested to be $\gamma$-good with respect to $f, \cD_\lambda$. 
%with input testing distribution $\cD$
\end{definition}

\begin{remark}
We will denote $\{P_{R_i,f}, Q_{R_i,f}\}$ to be the controlled projection for quantum program $\P_i = (\sigma[R_i], \{U_{R_i, x}\}_{x \in [N]})$ for $i \in \{1,2\}$.
We will then denote $\{\ti_{R_i,\gamma}, I - \ti_{R_i,\gamma} \}$ to be the Threshold Implementation for $\{\ti_{\gamma}(P_{R_i,f}), I - \ti_{\gamma}(P_{R_i,f}) \}$.

To test the $\gamma$-goodness of programs $\P_1, \P_2$, one can perform projection  $\ti_{R_1,\gamma}$  on $\sigma[R_1]$ and then perform  $\ti_{R_2,\gamma}$ on $\sigma[R_2]$. The order can be switched without affecting the final result because $\ti_{R_1,\gamma} \otimes I_{R_2}$ and $I_{R_1} \otimes \ti_{R_2,\gamma}$ commute. 
\end{remark}

\begin{definition}[$\gamma$-Anti-Piracy-Security] 
A copy protection scheme for function family $\cF$ and distribution $\cD$ has $\gamma$-anti-piracy security, if for all $\lambda \in \N$, for any QPT adversary $\cA$,  there exists a negligible function $\negl(\cdot)$ such that the following holds: 
  \begin{align}
    \Pr\left[b = 0, b \gets \AG_{\cF, \cD, \gamma}^\cA(1^\lambda) \right]\leq \negl(\lambda)
    \end{align}
\end{definition}


\begin{remark}
Note the probability $\Pr[b = 0, b \gets \AG_{\cF, \cD, \gamma}^\cA(1^\lambda)] = \E_{f }\left[\Tr[ (\ti_{R_1, \gamma} \otimes \ti_{R_2, \gamma} ) \cdot \sigma ]\right]$.
%\E_{f \gets \cD_f.
We will sometimes denote the above expression $\Pr[b = 0, b \gets \AG_{\cF, \cD, \gamma}^\cA(1^\lambda)]$ as adversary $\cA$'s advantage $\adv_\cA$ in game $\AG_{\cF, \cD, \gamma}^\cA(1^\lambda)$.
\end{remark}


==> prelim_append.tex <==
\section{Crytography Primitives and Assumptions}
\label{app:crypto_prelim2}

\begin{define}[One-Way Functions]
\label{def:owf}
A family of functions $\cF: \{0,1\}^n \to \{0,1\}^*$ is one-way if $f \in \cF$ can be computed in (classical) probablistic polynomial time(PPT) and for any  non-uniform PPT adversary $A$,  there exists a negligible function $\negl$ for all $n \in \N$ such that:
$$
\Pr[A(f(x)) \in f^{-1}(f(x))] \leq \negl
$$


\end{define}

%\paragraph{Trapdoor Functions}






\begin{define}[Public-Key Encryption]
\label{def:pke}
A (classical) public-key encryption scheme $\pke$ consists of three probabilistic polynomial-time  algorithms:

\begin{itemize}
    \item $\keygen(1^n) \to (\sk, \pk):$ a randomized algorithm that  takes as input a security parameter $n$
, and generates a secret and public key pair $(\sk, \pk)$.

\item $\enc(m \in \cM, \pk) \to \ct:$ a randomized algorithm that takes in public key $\pk$ and a message $m$ from message space $\cM$, and generates a ciphertext $\ct$.

\item $\dec(\ct, \sk) \to m/\bot: $  takes as input a secret key $\sk$ and a ciphertext $\ct$, and outputs a message $m$ 
or a symbol $\bot$ for decryption failure.
\end{itemize}

A secure $\pke$ scheme should satisfy the following properties:
\begin{description}
\item[Correctness:] For any $n \in \N$,  the following holds for any $m \in \cM$: 
$$
\Pr[\dec(\sk,  \ct \gets \enc(\pk, m)) = m ] = 1 
$$
probability taken over the choice $(\sk, \pk) \gets \keygen(1^n)$.

\item[IND-CCA(CCA2) Security:] A PKE scheme is secure under (classical) indistinguishability chosen-ciphertext attack, if for every PPT adversary $\cA$ there exists a negligible function $\negl$ such that for all $n \in \N$, the following holds:

\begin{gather*}
    \Pr\left[\cA^{\dec(\sk, \cdot)}(\ct) = b :
      \begin{array}{cl}
        (\pk, \sk) \gets \keygen( 1^n) \\
        ((m_0,m_1) \in \cM) \gets \cA^{\dec(\sk, \cdot)}(1^n, \pk) \\
        b \gets \{0,1\}; \ct \gets \enc(\pk, m_b)
      \end{array}
    \right] \leq \dfrac{1}{2} + \negl,
  \end{gather*}
where $\cA^{\dec(\sk, \cdot)}$ denotes that $\cA$ has access to the decryption oracle; $\cA$ can query the oracle both before and after the challenge phase.
Note that $\cA$ cannot query the decryption oracle on the encryptions of challenge messages $m_0, m_1$. 


\end{description}

%\paragraph{Weak Quantum CCA Security: }


\end{define}

\begin{define}[Digital Signatures]  
\label{def:signature}
A (classical) public-key digital signature scheme
D consists of three probabilistic polynomial-time classical algorithms:

\begin{itemize}
    \item $\keygen(1^n) \to (\sk, \pk):$ takes as input a security parameter $n$
, and generates a secret and public key pair $(\sk, \pk)$.

\item $\sign(m, \sk) \to (m,\sigma):$  takes in secret key $\sk$ and a message $m$, and generates a signature $\sigma$.

\item $\ver(m, \sigma, \pk) \to 0/1: $ takes as input public key $\pk$, a message $m$, and a claimed signature $\sigma$, and outputs either 1 for accept
or 0 for reject.
\end{itemize}

A secure digital signature scheme should satisfy the following properties:
\begin{description}
\item[Verification Correctness:] For any $n \in \N$,  so that the following holds: 
$$
\Pr_{(\sk, \pk) \gets \keygen(1^n)}[\ver(\pk, m, \sign(\sk, m)) = \text{ 1}] = 1 
$$

%probability taken over  $(\sk, \pk) \gets \keygen(1^n)$

\item[Unforgeability:] Suppose a PPT adversary $\cA$ is given $q = \poly(n)$ number of valid signatures from a signing oracle $\cO_{\sign}$ on any message $\cA$ queries, and then $\cA$ gives a claimed signature $(\sigma^*, m^*)$ on $m^*$ not queried before; for any such PPT $\cA$, there exists a negligible function $\negl$ for all $n \in \N$ such that:
$$
\Pr_{(\sk, \pk) \gets \keygen(1^n)}[\ver(\pk, \sigma^*, m^*) = 1 : (\sigma^*, m^*) \gets \cA^{\cO_{\sign}}(1^n)] \leq \negl
$$

%any $(\sk, \pk) \gets \keygen(1^n)$
\end{description}

\end{define}

\begin{define}[Learning With Errors Problem] \label{def:lwe}
An $\lwe_{n,m,q,\chi}$ instance is as follows. Let $\Z_q$ be the additive group modulo a large integer $q$; $A \gets \Z^{n \times m}, s \gets \Z^{n }, e \gets \chi^m$ where $\chi$ is an error distribution over $\Z_q$. Given $(A, b = A^\top s + e )$, the search problem is to find $s$.

The decisional $\lwe_{n,m,q,\chi}$ is to distinguish between $(A, b = A^\top s + e )$ and $(A, u)$ where $u \xleftarrow[]{R} \Z_q$.

\end{define}

\subsubsection{Psedorandom Functions and Puncturable PRFs}


\subsubsection{Non-Interactive Zero-Knowledge}

\begin{define}[Non-Interactive Zero-Knowledge]
\label{def_nizk}

\end{define}

\begin{define}[simulation-extractable NIZK]
\label{def_senizk}

\end{define}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse
\begin{theorem}[Inner Product Adversary Method \cite{aaronson2012quantum}]
\label{thm:inner_prod}
Let $S(n)$ denotes the set of $n/2$ dimensional subspaces in $\F^n$. Let $\cal R$ be a symmetric, anti-reflexive relation on $S(n)$ such that each subspace in $S(n)$ is related to at least one other subspace. Suppose that initially $|\la \psi_{init}^A|\psi_{init}^B\ra|\ge c$ for all $(A,B)\in {\cal R}$, whereas at the end we need $\E_{(A,B)\in \cal R}[|\la \psi_f^A|\psi_f^B\ra|]\le d$. Then, any algorithm achieving that must make $\Omega\Big( (c-d)2^{n/2} \Big)$ oracle queries.
\end{theorem}


\begin{define}[\iO, Definition 6.1] An indistinguishability obfuscator $\iO$ for a circuit class $\{{\cal C}_{\lambda}\}$ is a PPT uniform algorithm satisfying the following conditions:
\begin{itemize}
    \item For any $C\in {\cal C}_\lambda$, $\iO(\lambda, C)(x)=C(x)$ for all inputs $x$.
    \item For all pairs of PPT adversaries $(Samp, D)$, if there exists a negligible function $\alpha$ such that 
    $$
    \Pr[\forall x,C_0(x)=C_1(x):(C_0,C_1,\sigma)\leftarrow Samp(\lambda)]>1-\alpha(\lambda)
    $$
    then there exists a negligible function $\beta$ such that 
    $$
    |\Pr[D(\sigma,\iO(\lambda,C_0))=1]-\Pr[D(\sigma,\iO(\lambda, C_1))=1]|<\beta(\lambda)
    $$
\end{itemize}

\end{define}

\begin{define}[$\shO$, Definition 6.2] A subspace hiding obfuscator (\shO) for a field $\F$ and dimension $d_0,d_1$ is a PPT algorithm $\shO$ such that:
\begin{itemize}
    \item Input: description of subspace $S\subseteq \F^n$ of dimension $d\in \{d_0,d_1\}$.
    \item Output: membership circuit $\hat{S}$ such that:
    $$
    \Pr[\hat{S}(x)=S(x)\forall x:\hat{S}\leftarrow \shO(S)]\ge 1-\negl.
    $$
    \item Security:  consider the following game between an adversary and a challenger:
    \begin{itemize}
        \item The adversary choose a subspace $S_0$ of dimension $d_0$ and send it to the challenger
        \item The challenger picks randomly a subspace $S_1$ of dimension $d_1$ such that $S_0\subseteq S_1$. It then runs $\hat{S}\leftarrow \shO(S_b)$ for a random bit $b$ and gives $\hat{S}$ to the adversary
        \item The adversary makes a guess $b'$ for $b$
    \end{itemize}
    For all PPT adversary ${\cal A}$,
    $$
    \Pr[{\cal A}(\hat{S})=b]\le \frac{1}{2}+\negl.
    $$
\end{itemize}

\end{define}
\fi
